IHT dies hard: Provable accelerated Iterative Hard Thresholding

We study --both in theory and practice-- the use of momentum motions in classic iterative hard thresholding (IHT) methods. By simply modifying plain IHT, we investigate its convergence behavior on convex optimization criteria with non-convex constraints, under standard assumptions. In diverse scenaria, we observe that acceleration in IHT leads to significant improvements, compared to state of the art projected gradient descent and Frank-Wolfe variants. As a byproduct of our inspection, we study the impact of selecting the momentum parameter: similar to convex settings, two modes of behavior are observed --"rippling" and linear-- depending on the level of momentum.

==> proofs.tex <==
%!TEX root = AccIHT.tex

\section{Proof of Lemma \ref{thm:iter_inv}}{\label{sec:proofs}}

We start by observing that: $\|x_{i+1} - \bar{u}_i\|_2^2 \leq \|x^\star - \bar{u}_i \|_2^2$, due to the exactness of the hard thresholding operation.
Note that this holds for most $\mathcal{A}$ of interest\footnote{For example, in the case of matrices and low-rankness, this operation holds due to the Eckart-Young-Mirsky-Steward theorem, and the inner products of vectors naturally extend to the inner products over matrices.} but, again for simplicity, we will focus on the sparsity model here.
By adding and subtracting $x^\star$ and expanding the squares, we get:
\begin{align*}
\|x_{i+1} - x^\star + x^\star - \bar{u}_i\|_2^2 &\leq \|x^\star - \bar{u}_i \|_2^2 \Rightarrow \\
\|x_{i+1} - x^\star\|_2^2 + \|x^\star - \bar{u}_i\|_2^2 + 2 \left\langle x_{i+1} - x^\star, ~x^\star - \bar{u}_i \right \rangle &\leq \|x^\star - \bar{u}_i\|_2^2 \Rightarrow \\
\|x_{i+1} - x^\star\|_2^2 &\leq 2 \left \langle x_{i+1} - x^\star, ~\bar{u}_i - x^\star \right \rangle
\end{align*}

From the restricted strong convexity assumption over at most $4k$ sparse ``signals", we have:
\begin{align*}
f(x^\star) &\geq f(\bar{u}_i) + \left \langle \nabla f(\bar{u}_i), ~x^\star - \bar{u}_i \right \rangle + \tfrac{\alpha}{2} \|\bar{u}_i - x^\star\|_2^2 \Rightarrow \\
f(x^\star) - \tfrac{\alpha}{2} \|\bar{u}_i - x^\star\|_2^2 &\geq f(\bar{u}_i) + \left \langle \nabla f(\bar{u}_i), ~x^\star - \bar{u}_i \right \rangle \\
																		   &= f(\bar{u}_i) + \left \langle \nabla f(\bar{u}_i), ~x^\star - x_{i+1} + x_{i+1} - \bar{u}_i \right \rangle \\ 
																		   &= f(\bar{u}_i) + \left \langle \nabla f(\bar{u}_i), ~x_{i+1} - \bar{u}_i \right \rangle + \left \langle \nabla f(\bar{u}_i), ~x^\star - x_{i+1} \right \rangle 
\end{align*}
Define $\phi_i(z) := f(\bar{u}_i) + \left \langle \nabla f(\bar{u}_i), ~z - \bar{u}_i \right \rangle + \tfrac{\beta}{2} \|z - \bar{u}_i\|_2^2$.
Further, as claimed in Algorithm \ref{algo:alps}, we assume constant step size $\tfrac{\mu_i}{2} := \tfrac{1}{\beta}$, for all iterations $i$.
Then, it is easy to see that:
\begin{align*}
\min_{z:~\|z\|_{0, \mathcal{A}} \leq k} \phi_i(z) \equiv \min_{z:~\|z\|_{0, \mathcal{A}} \leq k} \tfrac{\beta}{2} \left \|z - \left(\bar{u}_i - \tfrac{1}{\beta} \nabla f(\bar{u}_i) \right) \right\|_2^2,
\end{align*} 
and thus, \emph{$x_{i+1}$ is the minimizer of $\phi_i(z)$ under $\mathcal{A}$ constraints}, by construction.

Let us denote the support of $x^\star$ as $\mathcal{X}^\star$. 
Further, denote as $\mathcal{E} := \mathcal{T}_i \cup \mathcal{X}^\star$. 
This implies that all the following hold: $(i)$ $u_i \in \mathcal{E}$, $(ii)$ $\bar{u}_i \in \mathcal{E}$, $(iii)$ $x^\star \in \mathcal{E}$, $(iv)$ $x_{i+1} \in \mathcal{E}$ and, $(v)$ the cardinality of $\mathcal{E}$ satisfies $|\mathcal{E}| \leq 4k$, where $k$ denotes the sparsity.
Denote $\mathcal{P}_{\mathcal{E}}(\cdot)$ the subspace projection operator (\emph{i.e.}, in the sparsity case it means that it keeps only the elements indexed by $\mathcal{E}$). 

By Remark 5.1(b) in \cite{beck2015minimization} and given that $x_{i+1}$ is a basic feasible point, the following holds\footnote{Remark 5.1(b) in \cite{beck2015minimization} claims that for a basic feasible point $x$ of a function $f(\cdot)$, it holds that: 
\begin{align*}
\left \langle \mathcal{P}_{\mathcal{E}}\left(\nabla f(x)\right), ~\mathcal{P}_{\mathcal{E}}\left(y - x\right) \right \rangle \geq 0, \quad \quad \text{for any}~~y \in \R^n \text{ such that } y \in \mathcal{E}.
\end{align*}
This holds for the most interesting cases for $\mathcal{A}$, such as sparsity, overlapping group sparsity and low-rankness, after modifications from vector to matrix case.}:
\begin{align*}
\left \langle \nabla \phi_i(x_{i+1}),~ x^\star - x_{i+1} \right \rangle &= \left \langle \nabla \phi_i(x_{i+1}),~ \mathcal{P}_{\mathcal{E}} \left(x^\star - x_{i+1}\right) \right \rangle \\
																						   &= \left \langle \mathcal{P}_{\mathcal{E}}\left(\nabla \phi_i(x_{i+1})\right),~ \mathcal{P}_{\mathcal{E}} \left(x^\star - x_{i+1}\right) \right \rangle \geq 0
\end{align*}
By the definition of $\phi_i(z)$, the above inequality leads to:
\begin{align*}
\left \langle \mathcal{P}_{\mathcal{E}}\left(\nabla f(\bar{u}_i) + \beta \left(x_{i+1} - \bar{u}_i\right)\right), ~\mathcal{P}_{\mathcal{E}}\left(x^\star - x_{i+1}\right) \right \rangle &\geq 0 \Rightarrow \\
\left \langle \mathcal{P}_{\mathcal{E}}\left(\nabla f(\bar{u}_i)\right), ~\mathcal{P}_{\mathcal{E}}\left(x^\star - x_{i+1}\right) \right \rangle &\geq \beta \cdot \left \langle \mathcal{P}_{\mathcal{E}}\left(x_{i+1} - \bar{u}_i \right), ~\mathcal{P}_{\mathcal{E}}\left(x_{i+1} - x^\star\right) \right \rangle \Rightarrow \\
\left \langle \nabla f(\bar{u}_i), ~x^\star - x_{i+1} \right \rangle &\geq \beta \cdot \left \langle x_{i+1} - \bar{u}_i, ~x_{i+1} - x^\star \right \rangle
\end{align*} 
where the last step is true due to all $x^\star, ~x_{i+1}$ and $\bar{u}_i$ belonging into the set $\mathcal{E}$.

Going back to the restricted strong convexity inequality, we use the above inequality to get:
\begin{align*}
f(x^\star) - \tfrac{\alpha}{2} \|\bar{u}_i - x^\star\|_2^2 &\geq f(\bar{u}_i) + \left \langle \nabla f(\bar{u}_i), ~x_{i+1} - \bar{u}_i \right \rangle + \beta \left \langle \bar{u}_i - x_{i+1}, ~x^\star - x_{i+1} \right \rangle \\
																		  &= \phi_i(x_{i+1}) - \tfrac{\beta}{2} \|x_{i+1} - \bar{u}_i\|_2^2 + \beta \left \langle \bar{u}_i - x_{i+1}, ~x^\star - x_{i+1} \right \rangle \\
																		  &= \phi_i(x_{i+1}) - \tfrac{\beta}{2} \|x_{i+1} - \bar{u}_i\|_2^2 + \beta \left \langle \bar{u}_i - x_{i+1}, ~x^\star - x_{i+1} + \bar{u}_i - \bar{u}_i \right \rangle \\
																		  &= \phi_i(x_{i+1}) - \tfrac{\beta}{2} \|x_{i+1} - \bar{u}_i\|_2^2 + \beta \left \langle \bar{u}_i - x_{i+1}, ~x^\star -  \bar{u}_i \right \rangle + \beta \|\bar{u}_i - x_{i+1}\|_2^2 \\
																		  &= \phi_i(x_{i+1}) + \tfrac{\beta}{2} \|x_{i+1} - \bar{u}_i\|_2^2 + \beta \left \langle \bar{u}_i - x_{i+1}, ~x^\star -  \bar{u}_i \right \rangle \\ 
																		  &\geq f(x^\star) + \tfrac{\beta}{2} \|x_{i+1} - \bar{u}_i\|_2^2 + \beta \left \langle \bar{u}_i - x_{i+1}, ~x^\star -  \bar{u}_i \right \rangle
\end{align*}
The last inequality is due to: $\phi_i(x_{i+1}) = f(\bar{u}_i) + \left \langle \nabla f(\bar{u}_i), ~x_{i+1} - \bar{u}_i \right \rangle + \tfrac{\beta}{2} \|x_{i+1} - \bar{u}_i\|_2^2 \geq f(x_{i+1}) \geq f(x^\star)$.
Thus:
\begin{align*}
- \tfrac{\alpha}{2} \|\bar{u}_i - x^\star\|_2^2 &\geq \tfrac{\beta}{2} \|x_{i+1} - \bar{u}_i\|_2^2 + \beta \left \langle \bar{u}_i - x_{i+1}, ~x^\star -  \bar{u}_i \right \rangle \Rightarrow \\
- \beta \left \langle \bar{u}_i - x_{i+1}, ~x^\star -  \bar{u}_i \right \rangle &\geq \tfrac{\beta}{2} \|x_{i+1} - \bar{u}_i\|_2^2 + \tfrac{\alpha}{2} \|\bar{u}_i - x^\star\|_2^2
\end{align*}

Going back to our initial inequality, we get:
\begin{align*}
\|x_{i+1} - x^\star\|_2^2 &\leq 2 \left \langle x_{i+1} - x^\star, ~\bar{u}_i - x^\star \right \rangle \\
                                     &= 2 \left \langle x_{i+1} - \bar{u}_i + \bar{u}_i - x^\star, ~\bar{u}_i - x^\star \right \rangle \\
                                     &= -2 \left \langle \bar{u}_i - x_{i+1}, ~\bar{u}_i - x^\star \right \rangle + \|\bar{u}_i - x^\star\|_2^2 \\
                                     &\leq - \|x_{i+1} - \bar{u}_i\|_2^2 - \tfrac{\alpha}{\beta} \|\bar{u}_i - x^\star\|_2^2 + \|\bar{u}_i - x^\star\|_2^2 \\
                                     &= \left(1 - \tfrac{\alpha}{\beta}\right) \|\bar{u}_i - x^\star\|_2^2 - \|x_{i + 1} - \bar{u}_i\|_2^2 \\
                                     &\leq \left(1 - \tfrac{\alpha}{\beta}\right) \|\bar{u}_i - x^\star\|_2^2
\end{align*}
To continue the proof, we need to expand the right hand side of the above expression:
\begin{align*}
\|\bar{u}_i - x^\star\|_2^2 &= \|u_i - \tfrac{1}{\beta} \nabla_{\mathcal{T}_i} f(u_i) - x^\star\|_2^2 \\
									&= \|u_i - x^\star\|_2^2 + \tfrac{1}{\beta^2} \|\nabla_{\mathcal{T}_i} f(u_i)\|_2^2 - 2 \left \langle \tfrac{1}{\beta} \nabla_{\mathcal{T}_i} f(u_i), ~u_i - x^\star \right \rangle 
\end{align*} 
and focus on the last term. 
In particular, we know that: $\left \langle \tfrac{1}{\beta} \nabla_{\mathcal{T}_i} f(u_i), ~u_i - x^\star \right \rangle  = \left \langle u_i - \bar{u}_i, ~ u_i - x^\star \right \rangle$. 
Using the same arguments as above, we can easily deduce that, by the strong convexity assumption, we have:
\begin{align*}
f(x^\star) - \tfrac{\alpha}{2} \|u_i - x^\star\|_2^2 \geq f(u_i) + \left \langle \nabla_{\mathcal{T}_i} f(u_i), ~x^\star - \bar{u}_i \right \rangle + \left \langle \nabla_{\mathcal{T}_i} f(u_i), ~\bar{u}_i - u_i \right \rangle
\end{align*}
Similarly to above, define function $h_i(z) := f(u_i) + \left \langle \nabla_{\mathcal{T}_i} f(u_i), ~z - u_i \right \rangle + \tfrac{\beta}{2} \|z - u_i\|_2^2 $, with minimizer the $\bar{u}_i$.  
Thus, by the optimality/feasibility conditions, we have:
\begin{align*}
\left \langle \nabla h(\bar{u}_i), ~x^\star - \bar{u}_i \right \rangle \geq 0 \Rightarrow \left \langle \nabla f(u_i), ~x^\star - \bar{u}_i \right \rangle \geq \beta \left \langle \bar{u}_i - x^\star, ~\bar{u}_i - u_i \right \rangle,
\end{align*}
and, therefore, following similar motions and under the assumption of Lemma \ref{thm:iter_inv} that $f(x^\star) \leq f(y)$, for any $y \in \R^\dim$ such that $\|y\|_{0, \mathcal{A}} \leq 3k$, we get:
\begin{align*}
\beta \langle u_i - \bar{u}_i, ~u_i - x^\star \rangle \geq \tfrac{\beta}{2} \|\bar{u}_i - u_i\|_2^2 + \tfrac{\alpha}{2} \|u_i - x^\star\|_2^2.
\end{align*}
We note that, while the assumption $\|y\|_{0, \mathcal{A}} \leq 3k$ is not necessarily mild, it does not restrict our analysis just to the noiseless setting.
It states that $x^\star$ has the minimum function value $f$, among all vectors that are at most $3k$-sparse. \emph{E.g.}, any dense vector, that might be a solution also due to noise, does not affect this requirement.

The above lead to:
\begin{align*}
\|x_{i+1} - x^\star\|_2^2 &\leq \left(1 - \tfrac{\alpha}{\beta}\right) \cdot \left(\|u_i - x^\star\|_2^2 + \tfrac{1}{\beta^2} \|\nabla_{\mathcal{T}_i} f(u_i)\|_2^2 - 2 \left \langle \tfrac{1}{\beta} \nabla_{\mathcal{T}_i} f(u_i), ~u_i - x^\star \right \rangle\right) \\
								  &\leq \left(1 - \tfrac{\alpha}{\beta}\right) \cdot \left(\|u_i - x^\star\|_2^2 + \tfrac{1}{\beta^2} \|\nabla_{\mathcal{T}_i} f(u_i)\|_2^2 - \|\bar{u}_i - u_i\|_2^2 - \tfrac{\alpha}{\beta} \|u_i - x^\star\|_2^2 \right) \\
								  &= \left(1 - \tfrac{\alpha}{\beta}\right)^2 \cdot \|u_i - x^\star\|_2^2
\end{align*}
Focusing on the norm term on RHS, we observe:
\begin{align*}
\|u_i - x^\star\|_2 &= \|x_i + \tau_i \left(x_i - x_{i-1}\right) - x^\star\|_2 = \|x_i + \tau_i \left(x_i - x_{i-1}\right) - (1 - \tau_i + \tau_i) x^\star\|_2 \\
						&= \|(1 + \tau_i)(x_i - x^\star) + \tau_i(x^\star - x_{i-1})\|_2 \\
						&\leq |1 + \tau| \cdot \|x_i - x^\star\|_2 + |\tau| \cdot \|x_{i-1} - x^\star\|_2
\end{align*} 
where in the last inequality we used the triangle inequality and the fact that $\tau_i = \tau$, for all $i$.
Substituting this in our main inequality, we get:
\begin{align*}
\|x_{i+1} - x^\star\|_2 &\leq \left(1 - \tfrac{\alpha}{\beta}\right) \cdot \left( |1 + \tau| \cdot \|x_i - x^\star\|_2 + |\tau| \cdot \|x_{i-1} - x^\star\|_2 \right) \\
							  &= \left(1 - \tfrac{\alpha}{\beta}\right) \cdot |1 + \tau| \cdot \|x_i - x^\star\|_2 + \left(1 - \tfrac{\alpha}{\beta}\right) \cdot |\tau| \cdot \|x_{i-1} - x^\star\|_2 
\end{align*}
Define $z(i) = \|x_i - x^\star\|_2$; this leads to the following second-order linear system:
\begin{align*}
z(i+1) \leq \left(1 - \tfrac{\alpha}{\beta}\right) \cdot |1 + \tau| \cdot  z(i) + \left(1 - \tfrac{\alpha}{\beta}\right) \cdot  |\tau| \cdot  z(i-1).
\end{align*}
We can convert this second-order linear system into a two-dimensional first-order system, where the variables of the linear system are multi-dimensional. 
To do this, we define a new state variable $w(i)$:
\begin{align*}
w(i) := z(i+1)
\end{align*} 
and thus $w(i+1) = z(i+2)$.
Using $w(i)$, we define the following 2-dimensional, first-order system:
\begin{align*}
\left\{
	\begin{array}{ll}
		w(i) - \left(1 - \tfrac{\alpha}{\beta}\right) \cdot |1 + \tau| \cdot  w(i-1) - \left(1 - \tfrac{\alpha}{\beta}\right) \cdot  |\tau| \cdot  z(i-1) \leq 0, \\
		z(i) \leq w(i-1).
	\end{array}
\right.
\end{align*}
This further characterizes the evolution of two state variables, $\{ w(i), z(i) \}$:
\begin{align*}
\begin{bmatrix}
w(i) \\ z(i)
\end{bmatrix} &\leq
\begin{bmatrix}
\left(1 - \tfrac{\alpha}{\beta}\right) \cdot |1 + \tau| & \left(1 - \tfrac{\alpha}{\beta}\right) \cdot  |\tau| \\
1 & 0
\end{bmatrix} \cdot 
\begin{bmatrix}
w(i-1) \\
z(i-1)
\end{bmatrix} \Rightarrow \\
\begin{bmatrix}
\|x_{i+1} - x^\star\|_2 \\ \|x_i - x^\star\|_2
\end{bmatrix} &\leq \begin{bmatrix}
\left(1 - \tfrac{\alpha}{\beta}\right) \cdot |1 + \tau| & \left(1 - \tfrac{\alpha}{\beta}\right) \cdot  |\tau| \\
1 & 0
\end{bmatrix} \cdot 
\begin{bmatrix}
\|x_i - x^\star\|_2 \\
\|x_{i-1} - x^\star\|_2
\end{bmatrix},
\end{align*}
where in the last inequality we use the definitions $z(i) = \|x_i - x^\star\|_2$ and $w(i) = z(i+1)$.
Observe that the contraction matrix has non-negative values.
%By defining $y(i) = \begin{bmatrix} \|x_{i+1} - x^\star\|_2 \\ \|x_i - x^\star\|_2 \end{bmatrix} $ and after unfolding the recursion over time, we obtain:
%\begin{align*}
%y(i+1) \leq \underbrace{\begin{bmatrix}
%\left(1 - \tfrac{\alpha}{\beta}\right) \cdot (1 + \tau) & \left(1 - \tfrac{\alpha}{\beta}\right) \cdot  \tau \\
%1 & 0
%\end{bmatrix}^i}_{:=A^i} \cdot y(0)
%\end{align*} 
This completes the proof.
